Data-Driven Reachability Analysis Using Matrix Zonotopes

In this paper, we propose a data-driven reachability analysis approach for unknown system dynamics. Reachability analysis is an essential tool for guaranteeing safety properties. However, most current reachability analysis heavily relies on the existence of a suitable system model, which is often not directly available in practice. We instead propose a data-driven reachability analysis approach from noisy data. More specifically, we first provide an algorithm for over-approximating the reachable set of a linear time-invariant system using matrix zonotopes. Then we introduce an extension for Lipschitz nonlinear systems. We provide theoretical guarantees in both cases. Numerical examples show the potential and applicability of the introduced methods.

==> Sections/4-reach_measnoise.tex <==

%\subsection{Measurement Noise} 
%\label{sec:measnoise}
In the following, we consider the case of measurement noise in addition to process noise, i.e., %i.e. while the system dynamics are described in \eqref{eq:sys}, we only have access to the noise-corrupted
\begin{align}
\begin{split}
    x(k+1) &= A x(k) + B u(k) + w(k),\\
    \tilde{x}(k) &= x(k) + v(k),
    \end{split}
    \label{eq:sys_v}
\end{align}
where $\tilde{x}(k)$, is the measured state that is additionally corrupted by measurement noise $v(k) \in \mathcal{Z}_v$.
Besides the input data matrix $U_-$, we analogously represent the state measurements by
\begin{align*}
    \tilde{X}_- &:= \begin{bmatrix} \tilde{x}(0) & \tilde{x}(1) & \dots & \tilde{x}(T-1)
    \end{bmatrix},     \\
    \tilde{X}_+ &:= \begin{bmatrix} \tilde{x}(1) & \tilde{x}(2) & \dots & \tilde{x}(T)
    \end{bmatrix}.
\end{align*}
%together with the input data matrix $U_-$ as before.
%We then only have access to the input sequence $\{u_k\}_{k=0}^{N-1}$ and measurements of the state that are additionally corrupted by measurement noise $\{\tilde{x}_k\}_{k=0}^{N}$.

Additionally, let $\hat{O} := \hat{V}_+ - A \hat{V}_-$ with
%Again, we denote the actual noise sequence that led to the data by $\{\hat{v}\}_{k=0}^{N}$ and $\{\hat{w}\}_{k=0}^{N-1}$. 
\begin{align*}
    \hat{V}_- &:= \begin{bmatrix} \hat{v}(0) & \hat{v}(1) & \dots & \hat{v}(T-1)
    \end{bmatrix},     \\
    \hat{V}_+ &:= \begin{bmatrix} \hat{v}(1) & \hat{v}(2) & \dots & \hat{v}(T)
    \end{bmatrix},
    %T_- := \begin{bmatrix} I_{N-1} \\ 0{1 \times N-1} \end{bmatrix} \\
    %T_+ := \begin{bmatrix} 0{1 \times N-1} \\ I_{N-1} \end{bmatrix} 
\end{align*}
where $\hat{v}(k)$, $k=0,1,\dots,T$, denotes again the actual measurement noise sequence that led to the measured input-state trajectories. Similar to the matrix zonotope $\mathcal{M}_w$ of the modeling noise, we have $\mathcal{M}_v=\zono{C_{\mathcal{M}_v},\tilde{G}_{\mathcal{M}_v}}$ where $\hat{V}_+,\hat{V}_- \in \mathcal{M}_v$. If we assume a knowledge of the bound on $\hat{O}$, the same approach as presented before can be pursued.
%\begin{align*}
%    \tilde{X}_+ - \hat{V} T_+ = A (\tilde{X}_- - \hat{V} T_-) + B U_- + W.
%\end{align*}


\begin{assumption}
\label{as:mmt_noise}
The matrix $\hat{O}$ is bounded by a matrix zonotope $\hat{O} \in \mathcal{M}_o$.    
%$\mathcal{M}_o = \langle C_o, G_o \rangle$.
\end{assumption}
\begin{proposition}
Given input $u(k)$ and state measurements $\tilde{x}(k)$, $k=0,1,\dots,T-1$, of the system in \eqref{eq:sys_v} and If there exists a matrix $\tilde{H}$ such that
\begin{align*}
    \begin{bmatrix} 
    \tilde{X}_- \\ U_- 
    \end{bmatrix} \tilde{H} = I
\end{align*}
then \begin{align*}
\hat{\mathcal{R}}_{i+1} = \mathcal{M}_{\tilde{\Sigma}} (\hat{\mathcal{R}}_{i} \times \mathcal{U}_i ) +  \mathcal{Z}_w, \quad \hat{\mathcal{R}}_{0}=\mathcal{X}_0
\end{align*}
with 
\begin{align*}
    \mathcal{M}_{\tilde{\Sigma}} = (\tilde{X}_+ - \mathcal{M}_o - \mathcal{M}_w) \tilde{H}
\end{align*}
contains the true model-based reachable set $\mathcal{R}_{i} \subset  \hat{\mathcal{R}}_{i}$. 
\end{proposition}
\begin{proof}
With
\begin{align*}
    \tilde{X}_+ - (\hat{V}_+ - A \hat{V}_-) - \hat{W} = A \tilde{X}_- + B U_-,
\end{align*}
 the proof follows the proofs of Theorem~\ref{th:reachdis} and Theorem~\ref{th:reach_lin} given Assumption~\ref{as:mmt_noise}.
\end{proof}
%\begin{align*}
%   \mathcal{M}_\Sigma = (\tilde{X}_+ - \mathcal{M}_R - \mathcal{M}_w) H.
%\end{align*}
%Write this as a lemma? Corollary? With this result, all methods and results of the remaining paper can be extended to the case where process as well as measurement noise exists. 
%
Note that a similar assumption to Assumption~\ref{as:mmt_noise} has been taken in \cite[Asm.~2]{conf:formulas}. However, it might be difficult in practice to find a suitable set $\mathcal{M}_o$ even with a given bound on $\hat{v}(k)$, $k=0,1,\dots,T$, since $A$ is assumed to be unknown. In the following, we introduce a practical approach, how an estimate on an over-approximation can be obtained. The general idea can be described as follows:

% One possible approach to over-approximate $\hat{O}$ in order to find a suitable set $\mathcal{M}_o$ is by an upper bound on the matrix norm of $A$. We denote $\lambda_{\max}$ as the largest absolute eigenvalue of $A$, i.e. $\lambda_{\max} = \max_i | \lambda_i (A)|$. Then, if $\hat{v}(k) \in \mathcal{Z}_v$ with $\mathcal{Z}_v = \langle C_{\mathcal{M}_v}, G_v \rangle$, the following holds:
% \begin{align*}
%     %\mathcal{M}_o = \mathcal{M}_v - \lambda_{\max} \mathcal{M}_v,
%     \hat{o}(k) \in \mathcal{Z}_v - [-\lambda_{\max}, \lambda_{\max}]  \mathcal{Z}_v.
% \end{align*}
% \tb{How is the correct notation here?}
% %where $\mathcal{M}_v$ is the matrix zonotope containing $\hat{V}_-$, $\hat{V}_+$. 
% This can then be used to deduce a zonotope $\mathcal{M}_o$ containing $\hat{O}$, which, however, might lead to conservative result. 


% , we define an approximate LTI model 
% \begin{align*}
%     \bar{\mathcal{M}}_{\tilde{\Sigma}} = (X_+ - \mathcal{M}_w) \tilde{H}
% \end{align*}
% for which
% \begin{align*}
%     \mathcal{M}_{\tilde{\Sigma}} = \bar{\mathcal{M}}_{\tilde{\Sigma}} - \mathcal{M}_o \tilde{H}.
% \end{align*}
% We hence know \tb{I think notation is wrong here, we can discuss on Monday}
% \begin{align*}
%   \bar{\mathcal{M}}_{\tilde{\Sigma}} \begin{bmatrix} \tilde{X}_- \\ U \end{bmatrix} - \mathcal{M}_{\tilde{\Sigma}} \begin{bmatrix} \tilde{X}_- \\ U \end{bmatrix}  \in \mathcal{M}_o
% \end{align*}
% We can calculate $\bar{\mathcal{M}}_{\tilde{\Sigma}} \begin{bmatrix} \tilde{X}_- \\ U \end{bmatrix}$, and we can approximate 
% \begin{align*}
%     \mathcal{M}_{\tilde{\Sigma}} \begin{bmatrix} \tilde{X}_- \\ U \end{bmatrix} \approx 
%     \mathcal{M}_{\tilde{\Sigma}} \begin{bmatrix} X_- \\ U \end{bmatrix} = \tilde{X}_+ - \mathcal{M}_v - \mathcal{M}_w.
% \end{align*}
% \tb{Whether we want to use the above or not is up for discussion, but I think it shows the difficulty in proving anything due to the approximation step}


% We propose another approach which assume the following assumption
%
% \begin{assumption}
% \label{assm:avuperbound}
% The data $\mathcal{D}$ contains the upper bound on the term $AV_-$. 
% \end{assumption}
%Our approach can summarized in the following two steps:
%


%Let $z(k) = \begin{pmatrix} x(k) \\ u(k) \end{pmatrix$.  denote the $i$-th column of $\begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix}$. 
%In the following, we introduce a practical approach, how an estimate on an over-approximation can be obtained. The general idea can be described as follows: %In the following, we present one approach to receive an estimate of $AV_-$ from data, which can be summarized as follows:

\begin{enumerate}
    \item Obtain an approximate model $M'$ while neglecting the term $A\hat{V}_-$.
    \item Obtain a zonotope that gives an over-approximation of the model mismatch, between the true model and the approximate model $M'$, and the term $A\hat{V}_-$ from data.
\end{enumerate}

To obtain an approximate model, we first neglect the term $A \hat{V}_-$, then use a least-squares approach 
\begin{align}
    M' = (\tilde{X}_+ - C_{\mathcal{M}_v} - C_{\mathcal{M}_w}  )\tilde{H}
    \label{eq:Mdash}
\end{align}
%where 
% \begin{align}
%    \begin{bmatrix} 
%    \tilde{X}_{-} \\ U_{-} 
%    \end{bmatrix} D' = I,
%    \label{eq:cond2dash}
%\end{align}
with the assumption that the right-inverse $\tilde{H}$ exists. Rewriting \eqref{eq:sys_v} in terms of the available data results in
\begin{align}
    \tilde{X}_+ - \hat{V}_+ = (M' + \Delta M') \begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} - A \hat{V}_- + \hat{W}_-, \label{eq:xpvp}
\end{align}
%where $\Delta M'$ is the model mismatch, i.e., $\Delta M' =\begin{bmatrix}A & B \end{bmatrix} - M'$. Given that $\hat{V}_+ \in \mathcal{M}_v$ and $\hat{W}_- \in \mathcal{M}_w$, we can find a matrix zonotope $\mathcal{M}_{AV}$ where $- A \hat{V}_- + \Delta M'\begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} \in \mathcal{M}_{AV}$ as following
where $\Delta M'$ is the model mismatch, i.e., $\Delta M' =\begin{bmatrix}A & B \end{bmatrix} - M'$. Rearranging \eqref{eq:xpvp} 
to have the unknown terms on the left-hand side results in 
\begin{align}
 \Delta M' \begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} - A \hat{V}_- =  \tilde{X}_+ - M'\begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} -  \hat{W}_- - \hat{V}_+   . \label{eq:xpvp}
\end{align}
We can find a matrix zonotope $\mathcal{M}_{AV}$, with $\Delta M'\begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} - A \hat{V}_-  \in \mathcal{M}_{AV}$, by replacing $\hat{V}_+$ by its enclosing set $\hat{V}_+ \in \mathcal{M}_v$ and similarly for $\hat{W}_- \in \mathcal{M}_w$. Then, $\mathcal{M}_{AV}$ can be computed as following
\begin{align}
\mathcal{M}_{AV} &= \tilde{X}_{+}- M' \begin{bmatrix}\tilde{X}_{-}\\ U_{-} \end{bmatrix} - \mathcal{M}_w  - \mathcal{M}_v.\label{eq:MAV}
\end{align}

We aim to find a zonotope $\mathcal{Z}_{AV}$ such that, $\forall j = 0,...,T-1$,
\begin{align}
 {(\tilde{X}_{+})}_{.,j} - M' \begin{bmatrix}{(\tilde{X}_{-})}_{.,j}\\ {(U_{-})}_{.,j} \end{bmatrix} -  {(\hat{W}_-)}_{.,j} - {(\hat{V}_+)}_{.,j} \in \mathcal{Z}_{AV}. \label{eq:ZAV}
\end{align}

%We can find an estimate on the upper and lower bounds on the terms $- A \hat{V}_- +  \Delta M' \begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix}$ by obtaining a matrix zonotope $\mathcal{M}_{AV}$ which captures the difference between applying the approximate model $M'$ on the data and true model captured in $\tilde{X}_{+}$, i.e.,

%
To do so we convert $\mathcal{M}_{AV}$ to an interval matrix \cite{conf:cora} and find the upper and lower bound along the horizontal dimension yielding:
\begin{align*}
[\underline{\mathcal{M}}_{AV} , \overline{\mathcal{M}}_{AV} ]&= \text{intervalMatrix}(\mathcal{M}_{AV}),\\
(\overline{\mathcal{Z}}_{AV})_i &= \argmaxB_j{(\overline{\mathcal{M}}_{AV})_{i,j}},\\ %\label{eq:argmaxMAV}\\
(\underline{\mathcal{Z}}_{AV})_i &= \argminB_j{(\underline{\mathcal{M}}_{AV})_{i,j}},\\ %\label{eq:argminMAV} \\
  \mathcal{Z}_{AV} &= \text{zonotope}(\underline{\mathcal{Z}}_{AV},\overline{\mathcal{Z}}_{AV}).
\end{align*}

%Rewriting \eqref{eq:xpvp} results in 
%\begin{align}
%    \tilde{X}_+ - \hat{V}_+ = M'  \begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} - A \hat{V}_- + \Delta M'\begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix}+ \mathcal{M}_w, \label{eq:xpvpv2}
%\end{align}

Given that $ \Delta M'\begin{bmatrix} {(\tilde{X}_-)}_{.,j} \\ {(U_-)}_{.,j} \end{bmatrix}- A {(\hat{V}_-)}_{.,j}  \in \mathcal{Z}_{AV}$, $\forall j =1, \dots, T$, and $X_+ = \tilde{X}_+ - V_+$, we rewrite \eqref{eq:xpvp} in terms of sets starting from $\hat{\mathcal{R}}_{0}=\mathcal{X}_0$ as follows
\begin{align}
\hat{\mathcal{R}}_{i+1} = M'\bigg( (\hat{\mathcal{R}}_i + \mathcal{Z}_v) \times \mathcal{U} \bigg) + \mathcal{Z}_{AV} +\mathcal{Z}_w. \label{eq:RAV}
\end{align}

\begin{remark}
The above approach provides a practical approach for computing the reachability analysis from noisy data (including process and measurement noise). In order to guarantee that the resulting reachability set is indeed an over-approximation of the true reachability set, one would need to assume that the data contains the upper and lower bounds on 
%We assume that the data is informative enough and contains upper and lower bounds on 
$  \Delta M' \begin{bmatrix} \tilde{X}_- \\ U_- \end{bmatrix} - A \hat{V}_- $. Mathematically speaking, we would require the availability of data points 
%$i_1, i_2 \in \mathbb{N}$, $i_1, i_2 \in [1,T]$, %
at some $k_1$ and $k_2$ for which  %$\hat{v}(k_1),z_{k_1}$, and $\hat{v}(k_2),z_{k_2}$ such that 
for which
\begin{align}
\Delta M' z(k_1) - A\hat{v}(k_1) \geq \Delta M' z - Av,\,\,\forall v\in \mathcal{Z}_v, z \in \mathcal{F}. \nonumber \\
\Delta M' z(k_2) - A\hat{v}(k_2) \leq \Delta M' z - Av,\,\,\forall v\in \mathcal{Z}_v, z \in \mathcal{F}. \nonumber 
\end{align} 
holds, where $z(k) = \begin{bmatrix} x(k) \\ u(k) \end{bmatrix}$.
However, even if this condition is not satisfied and no formal guarantees can be provided, the above approach showed its potential by over-approximating the reachable set in numerical examples.
\end{remark}

\begin{remark}
A similar approach can be used if we are interested in computing the reachable sets of continuous-time systems
\begin{align}
    \dot{x}(t) = A_c x(t) + B_c u(t) + w(t), 
    \label{eq:syscont}
\end{align} that are consistent with the noisy data sampled in discrete time. For this, we would need (noisy) measurements of the state as well as (noisy) measurements of the derivative of the state as done in \cite{conf:contin1,conf:contin2,conf:contin3}, as obtained, for example, via accelerator sensors. 
%\tb{I don't fully understand the following sentence. Maybe you can write even a bit more.} 
A similar approach to bound the model mismatch via a zonotope as described above can be used as set of models utilizing the traditional continuous time reachability analysis \cite{conf:thesisalthoff}. 
\end{remark}

%The following theorem summarizes computing the reachable set. Then find the upper and lower bounds on the horizontal dimension

%\begin{theorem}
%Given the data $\mathcal{D}$, the reachable set of \eqref{eq:sys_v} $\hat{\mathcal{R}}_{k} \supset \mathcal{R}_{k}$ starting from $\hat{\mathcal{R}}_{k}=\mathcal{X}_0$ can be computed as follows
%\begin{align}
%\hat{\mathcal{R}}_{k+1} = M'( \mathcal{R}_k \times \mathcal{U}_k ) + \mathcal{Z}_{AV} +\mathcal{Z}_w, \label{eq:RAV}
%\end{align}
%where
%\begin{align}
%  \mathcal{Z}_{AV} &= \text{zonotope}(\underline{\mathcal{Z}}_{AV},\overline{\mathcal{Z}}_{AV}), \\
%\overline{\mathcal{Z}}_{AV}(i) &= \argmaxB_j{\overline{\mathcal{M}}}_{AV}(i,j),\label{eq:argmaxMAV} \\ \underline{\mathcal{Z}}_{AV}(i) &= \argminB_j{\underline{\mathcal{M}}_{AV}(i,j)}, \label{eq:argminMAV}\\
%[\overline{\mathcal{M}}_{AV} , \underline{\mathcal{M}}_{AV} ]&= \text{intervalMatrix}(\mathcal{M}_{AV}),\\
%\mathcal{M}_{AV} &= X_{+} - \mathcal{M}_w - \tilde{M} \begin{bmatrix}X_{-}\\ U_{-} \end{bmatrix},\label{eq:MAV}
%\end{align}
%\tb{Again, $X$ is not available, right?}
%\end{theorem}

%\begin{proof}
%The approximated model in \eqref{eq:Mdash} is obtained by neglecting the term $AV_-$ and rearranging the following equation
%\begin{align}
%     \tilde{X}_+ - \hat{V}_+ =  A (\tilde{X}_- - \hat{V}_-) + B U_- + \hat{W}  ,
%\end{align}
% Given Assumption \ref{assm:avuperbound}, then the difference between the $X_+$ and applying the least square model $M'$ on the data $\mathcal{D}$ as shown in \eqref{eq:MAV} contains the upper-bound on the term $AV_-$ and the difference between the $M'$ and the true model \tb{as discussed last time and as also argued mathematically above, I doubt that this is true or that it can be shown without strong assumptions}. Thus, converting $\mathcal{M}_{AV}$ into interval matrix and finding the upper and lower bounds in \eqref{eq:argmaxMAV} and \eqref{eq:argminMAV} results in finding the required bounds. Converting the interval $(\underline{\mathcal{Z}}_{AV},\overline{\mathcal{Z}}_{AV})$ into zonotope $\mathcal{Z}_{AV}$ and adding that to the reachable region in \eqref{eq:RAV} assures that all states values are enclosed in  $\hat{\mathcal{R}}_{k+1}$.
%\end{proof}
%\tb{Don't you also need to account for the model mismatch?}

%Finding an improved (possibly non-conservative) approach in the case of measurement noise is a very challenging question, which is part of ongoing research.



==> Sections/5-reach_nonlin_V1.tex <==
\section{Reachability Analysis for Nonlinear Systems}\label{sec:reachnonlinear}

We consider an observable discrete-time nonlinear systems
\begin{align}
%\begin{split}
    x(k+1) &= f(x(k),u(k))+ w(k).
%\end{split}
    \label{eq:sysnonlin}
\end{align}

The local linearization of the nonlinear system \eqref{eq:sysnonlin} is performed by a Taylor series around linearization point $(x^*,u^*)$. Let $z(k)=\begin{bmatrix}x(k) \\u(k) \end{bmatrix}$. Then we use Taylor series as follows

\begin{align}
f(z) =& f(z^*) + \frac{\partial f(z)}{\partial z}\Big|_{z=z^*} (z - z^*) \nonumber\\
&+ \frac{1}{2}(z - z^*)^T \frac{\partial^2 f(z)}{\partial z^2}\Big|_{z=z^*}(z - z^*) + \dots
\end{align}

The infinite Taylor series can be over-approximated by a first order Taylor series and its Lagrange remainder $L$ \cite{conf:taylor}.

\begin{align}
f(z) \in & f(z^*) + \frac{\partial f(z)}{\partial z}\Big|_{z=z^*} (z - z^*) \nonumber\\
&+ \underbrace{\frac{1}{2}(z - z^*)^T \frac{\partial^2 f(\zeta)}{\partial z^2}\Big(z - z^*)}_{\text{Lagrange remainder} L}
\label{eq:linfL}
\end{align}
where
\begin{align}
\zeta \in \{ z^* + \alpha ( z-z^*) | \alpha \in [0,1] \}
\end{align}

We can rewrite \eqref{eq:linfL} as follows:

\begin{align}
f(x,u) \in & f(x^*,u^*) + \underbrace{\frac{\partial f(x,u)}{\partial x}\Big|_{x=x^*,u=u^*}}_{\tilde{A}} (x - x^*) \nonumber\\
&+ \underbrace{\frac{\partial f(x,u)}{\partial u}\Big|_{x=x^*,u=u^*}}_{\tilde{B}} (u - u^*) + L\nonumber\\
\in & \begin{bmatrix}f(x^*,u^*) & \tilde{A} & \tilde{B}\end{bmatrix} \begin{bmatrix}1\\x-x^*\\ u-u^*\end{bmatrix} +L
\end{align}

%In the following we assume that we sampled the data densely enough to infer bounds on the nonlinearity even in between data points.
The Lagrange remainder can be approximated by an interval which can be converted to a zonotope  \cite{conf:thesisalthoff}. 

Generally speaking, when dealing with data-driven methods for nonlinear systems, most works assume some form of continuity of the nonlinearity. Otherwise it is difficult task to generalize any system property of a nonlinear system from finite data. Continuity is often assumed in form of Lipschitz continuity on the the function $f(z)$ with a certain Lipschitz constant $L^\star$. Note that similar assumptions for data-driven analysis or control of nonlinear systems have been taken in~\cite{conf:montenbruckLipschitz,conf:novaraLipschitz}, where also estimation methods for the Lipschitz constant $L^\star$ from data are presented.  
\begin{assumption}
We the assume that $f(z)$ is Lipschitz continuous, i.e. that there is some $L^\star \geq 0$ such that the following inequality holds 
$$\| f(z_1) - f(z_2) \|_2 \leq L^\star \| z_1 - z_2\|_2 = \epsilon $$

\end{assumption}

%Then we can guarantee
%\begin{align}
%    f_{\mathrm{NL}}(z) \in \mathcal{Z}_{\mathrm{NL}} + \epsilon
%\end{align}
%with
%\begin{align}
%    \epsilon = L^\star \delta
%\end{align}
%when we have sampled densely ($x^\prime$: data points) : $\|x - x^\prime\|_2 \leq \delta$ for all $x \in \mathcal{X}_0$. ($\mathcal{X}_0$ or union of $\mathcal{X}_i$? tbd.)

%We assume that data stimulates all the non-linearity within $T$ time steps and 

We propose to compute data-driven reachability analysis for nonlinear system by the following two steps: 
\begin{enumerate}
    \item Obtain a set of approximative linearized models that are consistent with the noisy data.
    \item Obtain a zonotope that over-approximates Lagrange remainder for the chosen system. 
\end{enumerate}

%A set of linearized models which are consistent with noisy data according to the following theorem.


\begin{theorem}
\label{th:reachdisnonlin}
Given the system in \eqref{eq:sys}. If there exists a matrix $D$ such that 
\begin{align}
    \begin{pmatrix} 
    1\\ X_{-}-1 \otimes x^* \\ U_{-}-1 \otimes u^* 
    \end{pmatrix} D = I
    \label{eq:cond2}
\end{align}
reachable set computed based on the noisy data $\hat{\mathcal{R}}_{k} \supset \mathcal{R}_{k}$ starting from $\hat{\mathcal{R}}_{k}=\mathcal{X}_0$ can be computed as follows
\begin{align}
\hat{\mathcal{R}}_{k+1} = \mathcal{M}_{\Xi} (1 \times \hat{\mathcal{R}}_{k} \times \mathcal{U}_k) +  \mathcal{Z}_w +  \mathcal{Z}_L + \mathcal{Z}_\epsilon,
\end{align}
where
\begin{align}
 \mathcal{M}_\Xi &= (X_{+} - \mathcal{M}_w ) D \label{eq:zonoABnonlin} \\
\mathcal{Z}_L &= \text{zonotope}([\text{min}_{\leftarrow}(\mathcal{M}_L),\text{max}_{\leftarrow}(\mathcal{M}_L)]), \\
\mathcal{M}_L &= X_{+} - (\mathcal{M}_\Xi \begin{bmatrix}1\\X_{-}-1 \otimes x^*\\ U_{-}-1 \otimes u^*\end{bmatrix}\oplus \mathcal{M}_w ),\label{eq:zl} \\
\mathcal{Z}_\epsilon &= \zono{0,\text{diag}(\epsilon,\dots,\epsilon)}.
\end{align}
\end{theorem}

\begin{proof}
We have $W_- \in \mathcal{M}_w$ which can represented by considering specific $\beta_{W_-}$ that result in specific matrix inside the matrix zonotope $\mathcal{M}_w$:
\begin{align}
    W_- &= C_w + \beta_{W_-} G_w
    \label{eq:wzonononlin}
\end{align}
And we have from system model \eqref{eq:sysnonlin} while neglecting the Lagrange remainder $L$
\begin{align}
    W_{-} = X_{+} - \begin{bmatrix}f'(x^*,u^*) & \tilde{A}' & \tilde{B}'\end{bmatrix} \begin{bmatrix}1\\X_{-}-1 \otimes x^*\\ U_{-}-1 \otimes u^*\end{bmatrix}  
    \label{eq:wdatanonlin}
\end{align}
Equating \eqref{eq:wzonononlin} and \eqref{eq:wdatanonlin} yield
\begin{align}
C_w + \beta_{W_-} G_w = X_{+} - \begin{bmatrix}f'(x^*,u^*) & \tilde{A}' & \tilde{B}'\end{bmatrix} \begin{bmatrix}1\\X_{-}-1 \otimes x^*\\ U_{-}- 1 \otimes u^*\end{bmatrix}\!\! 
\label{eq:wzonowdatanonlin}
\end{align}

Rearranging \eqref{eq:wzonowdatanonlin} and considering all values for $-1 \leq \beta \leq 1$ instead of specific $\beta_{W_-}$ and given that the input is persistently exciting, we can arrive $\mathcal{M}_\Xi$ in \eqref{eq:zonoABnonlin}.
then the matrix zonotope that consider all possible $\begin{bmatrix}f'(x^*,u^*) & \tilde{A}' & \tilde{B}'\end{bmatrix} \in \mathcal{M}_\Xi$ can be found by
\begin{align}
   \mathcal{M}_\Xi = (X_{+} - \mathcal{M}_w ) D
    \label{eq:zonoABnonlin}
\end{align}
%where $\dagger$ is the pseudo inverse.   
Given that initial batch of data is informative enough about the non-linearity, We find the difference between data $X_{+}$ obtained by the nonlinear model and the our previously found linearized models applied on $U_{-}$ and $X_{-}$ as follows. %We find a data driven reachable region $\hat{\mathcal{R}}_{k}$ as an over approximation for the model based one $\mathcal{R}_{k}$ as follows
\begin{align}
\mathcal{M}_L &= X_{+} - (\mathcal{M}_\Xi \begin{bmatrix}1\\X_{-}-1 \otimes x^*\\ U_{-}-1 \otimes u^*\end{bmatrix}\oplus \mathcal{M}_w )
\end{align}
We note that $\mathcal{M}_L$ is matrix zonotope that maintains the difference between the nonlinear model and the linearized model for each data point. The matrix zonotope $\mathcal{M}_L$ over-approximates the linearization error for each data point. The next step is to find a zonotope that over-approximates the linearization error. This can done by converting $\mathcal{M}_L$ to matrix interval \cite{conf:cora}. Then find the upper-bound and the lower bound along the horizontal dimension $[\text{min}_{\leftarrow}(\mathcal{M}_L),\text{max}_{\leftarrow}(\mathcal{M}_L)]$. Given that the collected data stimulates all the nonlinearity for the system, then  $L \in [\text{min}(\mathcal{M}_L),\text{max}(\mathcal{M}_L)]$. Converting the resultant bound to a zonotope results in $\mathcal{Z}_L$. The final step is add $\mathcal{Z}_\epsilon$ to account for non-captured nonlinearity details in the data under the Lipschitz continuty assumption.
\end{proof}

%\tb{(We could use this in the proof and then in the example say it works well even if not sampled so densely?)}

%\tb{I think we should discuss once more what the advantage is to separate noise and nonlinearity? And whether to have local or global data...}





==> Sections/6-reach_cont.tex <==

\subsection{Reachability Analysis for Continuous-Time Systems}

%To do, I think
%\begin{itemize}
%\item Introduce why this is a very interesting problem (discrete time measurements, but system continuous time)
%\item Introduce exact discretization (+ assumptions, if applicable)
%\item Explain the logm operator + its series calculation
%\item Motivate why this is a hard problem
%\item State assumption
%\item State Theorem + Proof
%\item Short remark that calculating the series with the zonotope is also possible with guaranteed approximation error, but numerics have shown that the results are overly conservative?
%\end{itemize}

We are interested in computing the reachable sets of continuous time systems that are consistent with the data sampled in discrete time. Consider the following state space
\begin{align}
    \dot{x}(t) = A_c x(t) + B_c u(t) + w(t). 
    \label{eq:syscont}
\end{align}

%Measuring the current is type of measuring the derivativeof the voltage of the capacitor. Also, measuring the voltage of the inductor is kind of measuring the derivative of the current. The accelerometer sensor is measuring the derivative of the velocity as well. This approach can be summarized in the following theorem and is useful in certain applications. 

We propose two approaches to compute these reachable sets. First approach requires collecting the derivative of the signal as done in \cite{conf:contin1,conf:contin2,conf:contin3} and one example for that is the accelerator sensor. If we consider sampled noisy state derivative $\tilde{\dot{x}}(k)$ and noisy state, i.e.,
\begin{align}
\tilde{\dot{x}}(k) = \dot{x}(k) + g(k),\\
\tilde{x}(k) = x(k) + v(k),
\end{align}

where $g(k) \in \mathcal{Z}_g=\zono{c_g,G_g}$ and $v(k) \in \mathcal{Z}_v$ are bounded measurement noise. We collect $T$ data points  
\begin{align*}
    \tilde{\dot{X}} &:= \begin{bmatrix} \tilde{\dot{x}}(0) & \tilde{\dot{x}}(1) & \dots & \tilde{\dot{x}}(T-1) \end{bmatrix},
\end{align*}
with noise
\begin{align*}
 \hat{G} &:= \begin{bmatrix} \hat{g}(0) & \hat{g}(1) & \dots &\hat{g}(T-1) \end{bmatrix}.
\end{align*}

Similar to before, we have the noise in the collected data within a matrix zonotope, i.e., $G \in \mathcal{M}_g =\zono{C_{\mathcal{M}_g},G_{\mathcal{M}_g}^{(1:T)}}$. The problem is close the noisy measurement for discrete system with additional noise $g(k) \in \mathcal{Z}_g$ that affects the derivative of the data. We have for specific data points with actual noise $\hat{g}(k)$, $\hat{v}(k)$ and $\hat{w}(k)$:

\begin{align}
    (\tilde{\dot{X}})_i - \hat{g}(k) = \begin{bmatrix} A_c & B_c \end{bmatrix} \begin{bmatrix} (\tilde{X}_-)_i \\ (U)_i \end{bmatrix} - A_c \hat{v}(k) + w(k).
\end{align}

Again we first fit a model $M_c$ while neglecting the term $A_c \hat{v}(k)$ using least square as follows:
\begin{align}
    M_c = (\tilde{X}_+ - C_{\mathcal{M}_g} - C_{\mathcal{M}_w}  ) D_c
    \label{eq:Mc}
\end{align}
where 
 \begin{align}
    \begin{bmatrix} 
    \tilde{X}_{-} \\ U_{-} 
    \end{bmatrix} D_c = I,
    \label{eq:cond2Mc}
\end{align}
Then we find a zonotope $\mathcal{Z}_d$ that bounds the term $AV_-$ and the model mismatch, with the assumption  that the data is informative enough, as follows

\begin{align}
    \mathcal{M}_d &=\dot{X} - \mathcal{M}_w - \mathcal{M}_g - M_c \begin{bmatrix}X_{-} \\ U_{-} \end{bmatrix}.\label{eq:zc}
    \end{align}
Then obtain the upper and lower bound in a zonotope $\mathcal{Z}_d$ from $\mathcal{M}_d$ as in \eqref{eq:argmaxMAV} and \eqref{eq:argminMAV}.  
    
%    \begin{align}
%[\underline{\mathcal{M}}_d , \overline{\mathcal{M}}_d ]&= \text{intervalMatrix}(\mathcal{M}_d),\\
%(\overline{\mathcal{Z}_d})_i &= \argmaxB_j{(\overline{\mathcal{M}}_d)_{i,j}}, \\ (\underline{\mathcal{Z}_d})_i &= \argminB_j{(\underline{\mathcal{M}}_d)_{i,j}}, \\
%\mathcal{Z}_d &= \text{zonotope}(\underline{\mathcal{Z}}_d,\overline{\mathcal{Z}}_d). 
%\end{align}

Let $M_c =\begin{bmatrix} A_{M_c} & B_{M_c} \end{bmatrix}$. Then the next step is to use one of the readability analysis tool to find the reachable sets using the following parameters ($A_t$, $B_t$, $\mathcal{U}_t$, $\mathcal{X}_{t,0}$)
\begin{align}
 A_t &= A_{M_c}\\
 B_t & = 1 \\
 \mathcal{X}_{t,0} &= \mathcal{X}_{0} \\
 \mathcal{U}_t &= B_{M_c} \mathcal{U} + \mathcal{Z}_w +\mathcal{Z}_d
\end{align}

We consider the $\mathcal{Z}_w +\mathcal{Z}_d$ in $\mathcal{U}_t$ to be integrated along with the input. 

%\begin{theorem}
%Consider collected sampled data $\mathcal{D}$ from the system \eqref{eq:syscont}, the data-driven reachable set can be computed using traditional reachable techniques with the following parameters ($\mathcal{U}_c,\mathcal{A}_c,\mathcal{B}_c$)
%\begin{align}
% \mathcal{A}_c &= \mathcal{A}_{\Sigma,c}'\\
% \mathcal{B}_c & = 1 \\
% \mathcal{U}_c &= \mathcal{B}_{\Sigma,c}' \mathcal{U} + \mathcal{Z}_w +\mathcal{Z}_d
%\end{align}
%where
%\begin{align}
%\begin{bmatrix} 
%    X_- \\ U_- 
%\end{bmatrix} H &= I
%\end{align}
%\begin{align}
%\mathcal{M}_{\Sigma,c}' &= (\dot{X}_- - \mathcal{M}_w) H\\
%[ \mathcal{A}_{\Sigma,c}', \mathcal{B}_{\Sigma,c}'] &= \mathcal{M}_{\Sigma,c}'\\
%\mathcal{M}_d &=\dot{X}_- - \mathcal{M}_w - \mathcal{M}_{\Sigma,c} \begin{bmatrix}X_{-} \\ U_{-} \end{bmatrix},\label{eq:zc}\\
%[\overline{\mathcal{M}}_d , \underline{\mathcal{M}}_d ]&= \text{intervalMatrix}(\mathcal{M}_d),\\
%\overline{\mathcal{Z}_d}(i) &= \argmaxB_j{\overline{\mathcal{M}}_d(i,j)}, \\ \underline{\mathcal{Z}_d}(i) &= \argminB_j{\underline{\mathcal{M}}_d(i,j)}, \\
%\mathcal{Z}_d &= \text{zonotope}(\overline{\mathcal{Z}_d},\underline{\mathcal{Z}_d}), 
%\end{align}
%\end{theorem}



We propose another approach for data-driven reachability analysis for continuous time systems without requiring collecting the derivatives of the states. First of all, we assume that the discrete-time data points are obtained through zero-order hold inputs, which is the case in many application scenarios. Our approach is based on converting all the possible $\begin{bmatrix} A & B\end{bmatrix}$ in discrete time to continuous time. First we convert $\mathcal{M}_\Sigma$ to interval matrix which then bounds the all possible $\begin{bmatrix} A & B\end{bmatrix}$ as follows
\begin{align}
    [\underline{\mathcal{M}}_\Sigma,\overline{\mathcal{M}}_\Sigma ]&= intervalMatrix(\mathcal{M}_\Sigma) 
\end{align} 
 \begin{align}
   \underbrace{\begin{bmatrix}\underline{A} & \underline{B}\\ 0 & I\end{bmatrix}}_{\underline{D}} \leq \begin{bmatrix} A & B \\ 0 & I\end{bmatrix} \leq \underbrace{\begin{bmatrix} \overline{A} & \overline{B}   \\ 0 & I\end{bmatrix}}_{\overline{D}}
\end{align}  
where the operation $\leq$ is element wise. Let $\overline{D} = C_d + \Delta D_u$  and $\underline{D} = C_d - \Delta D_l$ where $C_d$ is any matrix between the bounds, i.e., $\underline{D} \leq C_d \leq \overline{D}$. The following theorem bounds all the possible $\begin{bmatrix} A_c & B_c\end{bmatrix}$ as follows: 

%Let $D_c :=  \begin{bmatrix} A_c & B_c \\ 0 & I\end{bmatrix}$, 

\begin{theorem}
Given the lower bounds $\begin{bmatrix}\underline{A} & \underline{B}\end{bmatrix}$ and upper bounds $\begin{bmatrix}\overline{A} & \overline{B}\end{bmatrix}$ on $\begin{bmatrix}A & B\end{bmatrix}$, we can bound $\begin{bmatrix}A_c & B_c\end{bmatrix}$ as follows
\begin{align}
   \begin{bmatrix} \underline{A}_c & \underline{B}_c \\ 0 & I\end{bmatrix} \leq  \begin{bmatrix} A_c & B_c \\ 0 & I\end{bmatrix}  \leq \begin{bmatrix} \overline{A}_c & \overline{B}_c \\ 0 & I\end{bmatrix}
\end{align}
\begin{align}
\begin{bmatrix} \overline{A}_c & \overline{B}_c \\ 0 & I\end{bmatrix} T_s&= \max(\log\begin{bmatrix} \overline{A} & \overline{B} \\ 0 & I\end{bmatrix},\log\begin{bmatrix} \underline{A} & \underline{B} \\ 0 & I\end{bmatrix})\\
\begin{bmatrix} \underline{A}_c & \underline{B}_c \\ 0 & I\end{bmatrix}T_s &= \min(\log\begin{bmatrix} \overline{A} & \overline{B} \\ 0 & I\end{bmatrix},\log\begin{bmatrix} \underline{A} & \underline{B} \\ 0 & I\end{bmatrix}),
\end{align}
where $T_s$ is the sampling time, $0 \leq \Delta D_l \leq 1$, $0 \leq\Delta D_u \leq 1$, $\Delta D_l \leq (C_d-I)$, $\Delta D_u \leq (C_d-I)$, and $C_d - I \leq 1$. The log is the matrix logarithm. The max, min and less than are element wise. 
\end{theorem}




\begin{proof}
We aim to prove that we can still bound $\begin{bmatrix} A_c & B_c \end{bmatrix}$ given the bounds in discrete time. Taking the logarithm of a matrix of $C_d$ and represented by power series.
\begin{align}
     log(C_d) &= \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(C_d - I)^k}{k}. \label{eq:cd}    %(C_d - I) - \frac{(C_d - I)(C_d - I)^T}{2}  +\dots
\end{align}
Considering $log(C_d +\Delta D)$ results in 
\begin{align}
log(C_d +\Delta D_u) =& \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(C_d  - I +\Delta D_u)^k}{k}\nonumber\\
=&  \sum_{k=1}^{\infty} \frac{(-1)^{k+1}}{k} \sum_{i=0}^{i}{k \choose i} (C_d  - I )^{k-i}\Delta D_u^i \label{eq:cddeltad}
%log(C_d +\Delta D) =& C_d +\Delta D - I - 0.5(C_d +\Delta D - I)^2 \nonumber\\
%&+ \frac{(C_d +\Delta D - I)^3}{3} - \frac{(C_d +\Delta D - I)^4}{4} + \dots \nonumber\\
%=&  C_d +\Delta D - I - 0.5 (C_d - I)^2 \nonumber\\
% - \Delta D (C_d  - I) - &0.5  \Delta D^2  + \frac{(C_d  - I)^3}{3} +  \Delta D(C_d  - I)^2 \nonumber\\ 
%+  \Delta D^2(C_d  - I) +& \frac{\Delta D^3}{3} - 0.25(C_d  - I)^4 - (C_d  - I)^3\Delta D \nonumber\\
%- 1.5(C_d  - I)^2&\Delta D^2 -  (C_d  - I)\Delta D^3 - 0.25 \Delta D^4 + \dots
\end{align}
Subtracting \eqref{eq:cd} from \eqref{eq:cddeltad} with denoting $h(\Delta D_u)= log(C_d +\Delta D_u) -  log(C_d)$ results in
\begin{align}
  h(\Delta D_u)\! =&\!\! \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k} \bigg(\! \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}\Delta D_u^i\! \nonumber\\ 
  &+ (C_d  -\! I )^k\! \bigg) -  \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k} (C_d  - I )^k \nonumber\\
   =& \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k}  \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}\Delta D_u^i\!
\end{align}
Similarly, we can find $h(-\Delta D)$ as
\begin{align}
h(-\Delta D_l)\! =  \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k}  \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}(-\Delta D_l)^i
\end{align}
Bounding the system dynamics in continuous time can be done by making sure that both $h(\Delta D_u)$ and $h(-\Delta D_l)$ do not increase or decrease together but one increases and the other decreases. 
%\begin{align}
%log(C_d + \Delta D) - log(C_d)&= \Delta D - \Delta D(C_d  - I) - 0.5\Delta D^2 \nonumber\\
%+ \Delta D (C_d  - I)^2 +&  (C_d  - I)\Delta D^2 + \frac{\Delta D^3}{3} \nonumber\\
%- (C_d  - I)^3\Delta D -& 1.5(C_d  - I)^2\Delta D^2 - (C_d  - I)\Delta D^3 \nonumber\\
%- \Delta D^4 + \dots&\\
%log(C_d - \Delta D) - log(C_d)&= -\Delta D + \Delta D(C_d  - I) - 0.5\Delta D^2 \nonumber\\
%- \Delta D (C_d  - I)^2 +&  (C_d  - I)\Delta D^2 - \frac{\Delta D^3}{3} \nonumber\\
%+ (C_d  - I)^3\Delta D -& 1.5(C_d  - I)^2\Delta D^2 + (C_d  - I)\Delta D^3 \nonumber\\
%- \Delta D^4 + \dots&
%\end{align}
Given that $0 \leq \Delta D_u \leq 1$, $0 \leq \Delta D_l\leq 1$ and $(C_d-I) \leq 1$, then the dominant terms are $\Delta D_u$ and $\Delta D_u(C_d  - I)$ (similarly with $\Delta D_l$) and they are with different signs for $h(\Delta D_u)$ and $h(-\Delta D_l)$. At odd  value of index $i$, the $h(\Delta D_u)$ and $h(-\Delta D_l)$ have difference sign which support our claim. For index $i$ equals even values, both $h(\Delta D_u)$ and $h(-\Delta D_l)$ have the same sign. However given that $\Delta D_l \leq (C_d-I)$ and $\Delta D_u \leq (C_d-I)$, then there is always a term at the same index $i$ with greater value. %For instance, the terms $(C_d  - I)\Delta D^2$, $1.5(C_d  - I)^2\Delta D^2$, and $\Delta D^4$ are smaller than the comparable terms in the series.  
\end{proof}





%Assume that even though we have discrete-time trajectories, the underlying system is in fact continuous time. To retrieve a reachability analysis also in between data points, we are therefore interested in finding a set of continuous time systems that are consistent with the data.

%First of all, we assume that the discrete-time data points are obtained through zero-order hold inputs, which is the case in many application scenarios. % (note: realistic assumption on actuator). (Remark: This could also be refined to ramp-invariant transformation)





%Second assumption, we assume that the sampling rate is satisfactory and the spectral norm of $AT_s $ satisfies the following inequality:
%\begin{align*}
%   \| A T_s \| \leq 0.5
%\end{align*}

%Then we know 
%\begin{align*}
%    A_{\mathrm{disc}} &= e^{AT_s} = I + AT_s + \frac{1}{2!}(A T_s)^2 + \dots \\
%    B_{\mathrm{disc}} &= \int_0^{T_s} e^{At} B dt = \left( I T_s + A T_s^2 + \frac{1}{2!}A^2 T_s^3 + \dots \right) B
%\end{align*}

%\begin{theorem}
%The approximation error can be bounded by 
%\begin{align*}
%    \| E_m \| \leq \frac{\rho (L) ^{m+1}}{(m+1)(1+\rho(L))}
%\end{align*}
%where $\rho(L)$ denotes the spectral radius of $L$.
%\end{theorem}
%\begin{proof}
% (Lastman, Puthenpura and Sinha 1984)
%\end{proof}

%\subsubsection*{Algorithm \cite{conf:bookdisc2cont}}
%\begin{enumerate}
%    \item Determine $L = A_{\mathrm{disc}} - I$.
%    \item Set $D^{(1)} = I$, $M^{(1)} = I$ and $i=1$.
%    \item Perform the following computations recursively
%    \begin{align*}
%        M^{(i+1)} &= \frac{-i L M^{(i)}}{i+1} \\
%        D^{(i+1)} &= D^{(i)} + M^{(i+1)} \\
%        i &= i+1
%    \end{align*}
%    until $i=m$.
%    \item Finally, $AT = DL$, $BT = D B_{\mathrm{disc}}$
%\end{enumerate}



% This is what we need!
% https://link.springer.com/content/pdf/10.1007%2F978-94-011-3558-0.pdf p.131

%A method to calculate \cite{conf:disc2cont}, but calculations are involved and not tractable for matrix zonotopes. However, we can calculate the Euler approximation and then bound the local truncation error?

% Can we use this? "TRANSFORMATION OF CONTINUOUS-TIME MODEL OF A LINEAR MULTIVARIABLE SYSTEM FROM ITS DISCRETE-TIME MODEL"

%\tb{no results here - just thoughts we can discuss}
%$\rightarrow$ How can we find the continuous time state space description?
%Assuming zero-order hold for the input (I think a good choice), we retrieve
%\begin{align*}
%    A_{\text{disc}} = e^{AT_s}
%\end{align*}
%with $T_s$ being the sampling time. However, calculating the logarithm of a matrix is usually done via diagonalization. If $\|A_{\text{disc}} - I \| < 1$ (what does that mean for us?), then it can be calculated the following series converges:
%\begin{align*}
%    A T_s = \log (A_{\mathrm{disc}}) = \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(A_{\mathrm{disc}} - I)^k}{k}
%\end{align*}
%..can we calculate this sum via Zonotopes? We can only be approximating the true matrix.

%..which is actually the Euler integration. For small timesteps $T_s$, $e^{A T_s} \approx I + A T_s $, i.e. $A T_s \approx A_{\mathrm{disc}} - I  \left( = \sum_{k=1}^{1} (-1)^{k+1} \frac{(A_{\mathrm{disc}} - I)^k}{k}\right)$, $B T_s \approx B_{\mathrm{disc}}$. % $D_{\mathrm{disc}} = D$, $C_{\mathrm{disc}} = C$
% http://eceweb1.rutgers.edu/~gajic/solmanual/slides/chapter8_DIS.pdf
% https://homes.esat.kuleuven.be/~maapc/static/files/CACSD/Slides/chapter2.pdf

%I guess we can use Euler discretization for small timesteps - but we introduce an error. Can we bound the error? Then we could add this error in the reachability analysis. 

%The local error (error per step) is proportional to the square of the step size.
%Assume $x$ has a continuous second derivative. Local truncation error LTE:
%\begin{align*}
%    \mathrm{LTE} = \frac{1}{2} T_s^2 M 
%\end{align*}
%where $M$ is the an upper bound on the second derivative of $x$ on the given interval $[t_0, t_0 + h]$.

%\begin{align*}
%    \dot{x} &= Ax + Bu \\
%    \ddot{x} &= A \dot{x} = A^2 x + ABu
%\end{align*}
%While we cannot calculate the exact discretization error, we can approximate it by $A_{\mathrm{disc}}^2 x(t_0) + A_{\mathrm{disc}} B_{\mathrm{disc}} u(t_0)$? \tb{tbd}.





%Let $\mathcal{M}_{\Sigma} = \begin{bmatrix}\mathcal{M}_{\Sigma A} & \mathcal{M}_{\Sigma B} \end{bmatrix}$. The reachable region can be over approximated by 
%\begin{align}
%\mathcal{R}_{k+1} = \mathcal{M}_{\Sigma A} \mathcal{R}_{k} + \mathcal{M}_{\Sigma B} \mathcal{U} +  \mathcal{M}_w
%\end{align}
%
